A conservative discontinuous Galerkin scheme for the 2D incompressible Navier--Stokes equations

In this paper we consider a conservative discretization of the two-dimensional incompressible Navier--Stokes equations. We propose an extension of Arakawa's classical finite difference scheme for fluid flow in the vorticity-stream function formulation to a high order discontinuous Galerkin approximation. In addition, we show numerical simulations that demonstrate the accuracy of the scheme and verify the conservation properties, which are essential for long time integration. Furthermore, we discuss the massively parallel implementation on graphic processing units.

==> conservation.tex <==
\section{Conservation for Dirichlet boundary condition\label{sec:BC} } 
Based on the discussion in the previous two sections one might be tempted to conjecture that the constructed scheme is also conservative in the case of homogeneous Dirichlet boundary conditions (as opposed to periodic boundary conditions). That this is not true can be seen by the following argument.

Let us 

